Implementation of hyperspectral inversion algorithms on FPGA: Hardware comparison using High Level Synthesis

Hyperspectral imaging is gathering significant attention due to its potential in various domains such as geology, agriculture, ecology, and surveillance. However, the associated processing algorithms, which are essential for enhancing output quality and extracting relevant information, are often computationally intensive and have to deal with substantial data volumes. Our focus lies on reconfigurable hardware, particularly recent FPGAs. While FPGA design can be complex, High Level Synthesis (HLS) workflows have emerged as a solution, abstracting low-level design intricacies and enhancing productivity. Despite successful prior efforts using HLS for hyperspectral imaging acceleration, we lack a comprehensive research to benchmark various algorithms and architectures within a unified framework. This study aims to quantitatively evaluate performance across different inversion algorithms and design architectures, providing insights for optimal trade-offs for specific applications. We apply this analysis to the case study of spectrum reconstruction processed from interferometric acquisitions taken by Fourier transform spectrometers.

==> extra/fft_algorithm.tex <==
\subsubsection{\underline{\textbf{\ac{fft} algorithm}}}
\label{sec:fft-alg}

\textcolor{orange}{This should be known. Any parts/details of implementation that are original to this work? If so, they should be stated.}
\textcolor{red}{Agree.}

The Cooley-Tukey \ac{fft} algorithm~\cite{cooley1965algorithm} eliminates redundancy by separating the computation in alternating sequences in order to identify shared operations. For instance, by separating the original size $N$ \ac{dft} into \textit{even} and \textit{odd} samples and exploiting some twiddle factors' properties such as periodicity and symmetry of eq.\eqref{eq:twid_sym}, we end up with a combination of two \ac{dft}s of size $N/2$ of eq.\eqref{eq:dft_1}. This first partitioning (Fig.\ref{fig:first_parti_fft}) results in $(N^2/2+N)$ operations instead of $N^2$. This structure is called \textit{radix-2} as each stage is partitioned into two sequences.

\begin{equation}\label{eq:twid_sym}
\resizebox{0.91\hsize}{!}{$W_{N}^{k}=e^{\frac{-j2\pi}{N} k} \qquad W_{N}^{k(N+n)}=W_{N}^{kn} \qquad W_{N}^{k(N-n)}=W_{N}^{-kn}=(W_{N}^{kn})^*$}
\end{equation}

\begin{equation}\label{eq:dft_1}
\resizebox{0.91\hsize}{!}{$X_{k}=\sum_{n=0}^{N-1}x_{n}.W_{N}^{kn} \quad = \quad \underbrace{\sum_{m=0}^{N/2-1}x_{2m}.W_{N}^{2k}}_{\text{Even samples' DFT}} + W_{N}^{k}\underbrace{\sum_{m=0}^{N/2-1}x_{2m+1}.W_{N}^{2k}}_{\text{Odd samples' DFT}}$}
\end{equation}


The more deeply we partition, the faster the algorithm will be. This process is repeated up to reach a graph with only size 2 \ac{dft}s (Fig.\ref{fig:last_parti_fft}). At this point, all redundant operations would be eleminated. This partitioning is called \ac{dit} and it can also be performed over the outputs in \ac{dif}. The smallest indivisible \ac{dft} is called a butterfly. The computation graph is composed of $log_2{N}$ stages each composed of $\frac{N}{2}$ butterflies. For a $radix-R$ partitioning, the computation complexity would be of $\frac{N}{R}.log_R{N}$ complex operations, $log_R{N}$ stages and $\frac{N}{R}$ butterflies per stage.

\begin{figure}[!ht]
  \begin{center}
	\subfloat[First partitioning\label{fig:first_parti_fft}]{%
		\includegraphics[width=0.7\columnwidth]{figures/fft_principale_step1}
	}
	\hfill
	\subfloat[Last partitioning\label{fig:last_parti_fft}]{%
		\includegraphics[width=0.7\columnwidth]{figures/fft_principale_step3}
	}
	\caption{8 points example of $radix-2$ \ac{dit} \ac{fft} graph.}
	\label{fig:fft_parti}
  \end{center}
\end{figure}

==> extra/preamble.tex <==
\usepackage{acronym}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}
\usepackage{listings}
\usepackage{amsmath}
\usepackage{amsfonts}

\lstset{% 
    basicstyle=\small\ttfamily\bfseries,
    columns=flexible,
    language=SAS,
    keywordstyle=\color{black}\bfseries,
    morecomment=[s]{/*}{*/},
    morecomment=[s]{*}{;},
    morecomment=[n]{/*}{*/},
    morecomment=[n]{*}{;},
    escapechar=|,
    commentstyle=\color{green}\ttfamily,
    stringstyle=\color[rgb]{0.639,0.082,0.082}\ttfamily,
    showstringspaces=false,
    keepspaces=true,
    sensitive=false,
    otherkeywords={*,/},
}

\newenvironment{saslst}{\VerbatimEnvironment\noindent\begin{minipage}{\linewidth}\begin{lstlisting}}
 {\end{lstlisting}\end{minipage}}
 
\usepackage{showexpl}
\newcommand{\range}[3]{#1\in[#2,...,#3]}



%%%%%%%%%%%%%%%%%%%%% acronym %%%%%%%%%%%%%%%%%%%%%%%%%%

\newacro{fft}[FFT]{fast Fourier transform}
\newacro{dft}[DFT]{discrete Fourier transform}
\newacro{dct}[DCT]{discrete cosine transform}
\newacro{dit}[DIT]{decimation-in-time}
\newacro{dif}[DIF]{decimation-in-frequency}
\newacro{dma}[DMA]{direct memory access}
\newacro{hls}[HLS]{high-level synthesis}
\newacro{rtl}[RTL]{register transfer level}
\newacro{fpga}[FPGA]{field-programmable gate array}
\newacro{asic}[ASIC]{application specific integrated circuit}
\newacro{ip}[IP]{integrated processor}
\newacro{fp}[FP]{floating point}
\newacro{fxp}[FxP]{fixed point}
\newacro{bfp}[BFP]{block floating point}
\newacro{pe}[PE]{processing element}
\newacro{mdc}[MDC]{multi-path delay commutator}
\newacro{sdc}[SDC]{single-path delay commutator}
\newacro{sdf}[SDF]{single-path delay feedback}
\newacro{snr}[SNR]{signal-to-noise ratio}
\newacro{ofdm}[OFDM]{orthogonal frequency-division multiplexing}
\newacro{dsp}[DSP]{digital signal processing}
\newacro{cem}[CEM]{constrained energy minimization}
\newacro{fts}[FTS]{Fourier Transform Spectrometer}
\newacro{svd}[SVD]{singular value decomposition}
\newacro{tsvd}[TSVD]{truncated singular value decomposition}
\newacro{pinv}[PINV]{pseudo-inverse}
\newacro{tik}[TIK]{Tikhonov regularization}
\newacro{fts}[FTS]{Fourier transform spectrometer}
\newacro{opd}[OPD]{optical path difference}
\newacro{sv}[s.v.]{singular value}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mdm}[1]{\textcolor{orange}{#1}}
\newcommand{\dapi}[1]{\textcolor{red}{#1}}
\newcommand{\sm}[1]{\textcolor{magenta}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> gfx/lat_freq_comp_obsolete.tex <==
\begin{figure}
    \begin{subfigure}[b]{0.49\linewidth}
        \input{gfx/lat_freq_comp_obsolete_1}
    \end{subfigure}

    \begin{subfigure}[b]{0.49\linewidth}
        \input{gfx/lat_freq_comp_obsolete_2}
    \end{subfigure}
\end{figure}

==> gfx/mm_fft_mono.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/mm_fft_main_bfp}
  \caption{multi banks, memory-based \ac{fft} architecture.}
  \label{fig:mm_fft_mono}
\end{figure}

==> gfx/rdx_PO_perf_compar.tex <==
\begin{table*}[!ht]
	\centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
      \hline
        &\textbf{R2 PR} & \textbf{R2 PO} & \textbf{R4 PR} & \textbf{R4 PO}\\
      \hline
      Operands Datawidth(bits) & 18 & 18 & 18 & 18\\
      Twiddles Datawidth(bits) & 18 & 18 & 18 & 18\\
      Precision & BFP & BFP & BFP & BFP\\
      \hline
      LUTs & 1048 & 1182 & 2638 & 1907\\
      FFs & 107 & 817 & 84 & 1387 \\
      BRAMs & 3 & 3 & 5 & 8\\
      DSPs & 4 & 4 & 12 & 12\\
      \hline
      Max Frequency ($Mhz$) & 68.17 & 209.64 & 62.61 & 203.99\\ % <-- added row here
      Latency cycles & 5126 & 5135 & 1282 & 1290\\
      Transform cycles & 5128 & 5137 & 1284 & 1293\\   
      \hline
    \end{tabular}
    
    \vspace{1mm}
    PR : Pre-Butterfly Shift / PO : Post-Butterfly Shift\\
    R2 : Radix 2 / R4 : Radix 4
    \vspace{2mm}
    \caption{Radix-2 and Radix-4 FFT implementation results and performance comparison.  \ac{bfp} performance comparison carried out by implementing 18bits precision, 1024 points FFT on Artix-7 technology using a memory-based HLS architecture.}
    \label{tab:rdx_PO_perf_compar}
\end{table*}	
